Reachability Analysis for Attributes in ABAC with Group Hierarchy

Attribute-based access control (ABAC) models are widely used to provide fine-grained and adaptable authorization based on the attributes of users, resources, and other relevant entities. Hierarchial group and attribute based access control (HGABAC) model was recently proposed which introduces the novel notion of attribute inheritance through group membership. GURAG was subsequently proposed to provide an administrative model for user attributes in HGABAC, building upon the ARBAC97 and GURA administrative models. The GURA model uses administrative roles to manage user attributes. The reachability problem for the GURA model is to determine what attributes a particular user can acquire, given a predefined set of administrative rules. This problem has been previously analyzed in the literature. In this paper, we study the user attribute reachability problem based on directly assigned attributes of the user and attributes inherited via group memberships. We first define a restricted form of GURAG, called rGURAG scheme, as a state transition system with multiple instances having different preconditions and provide reachability analysis for each of these schemes. In general, we show PSPACE-complete complexity for all rGURAG schemes. We further present polynomial time algorithms to solve special instances of rGURAG schemes under restricted conditions.

==> Images/Irrelevant/figure2.tex <==
\iffalse
\begin{figure}[t]
\centering
\includegraphics[scale=.55]{Images/Fig2-v2.png}
\caption{\rGURAG Schemes and Complexity Classes}
\label{fig:complexity}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=.55]{Images/Fig-complexity.png}
\caption{\rGURAG Schemes and Complexity Classes}
\label{fig:complexity}
\end{figure}
\begin{figure*}[t]
\centering
\includegraphics[scale=.70]{Images/Fig-complexity-v4.png}
\caption{\rGURAG Schemes and Complexity Classes}
\label{fig:complexity}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[scale=.75]{Images/Fig-complexity-v5.png}
\caption{\rGURAG Schemes and Complexity Classes}
\label{fig:complexity}
\end{figure*} \fi
\begin{figure*}[t]
\centering
\includegraphics[scale=.75]{Images/complexity-v1.png}
\caption{\rGURAG Schemes and Complexity Classes}
\label{fig:complexity}
\end{figure*}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/Irrelevant/algo-sa-1n.tex <==
\begin{algorithm*}[t]  \footnotesize
\centering
\caption{Plan Generation for \RPSAME in [\miniGURANGO -- $\overline{N}$]}
\label{algo:sa-1n}
\begin{algorithmic}[1]
\State{\textbf{Input:} problem instance I = $\langle$$\gamma_0$, $q$$\rangle$  \textbf{Output:} $plan$ or false}
\State{$plan$ := $\langle\rangle$;}
\Comment{\texttt{Initialize plan}}
\State{$s$ := $\gamma_0$;}
\Comment{\texttt{Initialize with state s}}
%\State{\textbf{if} $s$ $\vdash_{\RPSAME}$ $q$ \textbf{then}\textbf{return} $plan$}
\State{\textbf{if} ($\exists$ $att$ $\in$ \ATTR. $\exists$ $\mathrm{\langle}$$u$, $e\_{{att}}$, $vset$$\mathrm{\rangle}$ $\in$ $q$). $e\_att(u)$ $-$ $vset$ $\neq$ $\emptyset$ \textbf{then return} false;}
\Comment{\texttt{Check if state s has more values than query}}
% $\langle\rangle$}
%\While{$true$}
%\State{\textbf{Let} $Save$ = $\eUAAN_s$;}
\LeftComment{\texttt{ Assign attribute values required in query to the user or user's effective groups}}
\While{($s$ $\nvdash_{\RPSAME}$ $q$ $\land$ \State{((($\exists$ $att'$ := $att$ $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val \mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att'}$). ($\Evaluate_u(u,~c,~s)$
  $\wedge$ $val$ $\notin$ $att'$($u$) $\wedge$ $\exists$ $\mathrm{\langle}$$u$, $e\_{{att'}}$, $vset$$\mathrm{\rangle}$ 
  %$\langle$ $q$$_{e\_att'}$, $q$$_{e\_att'}$$(u)$ $\rangle$
  $\in$ $q$. $val$ $\in$ $vset$ ))} \State{$\lor$} \State{(($\exists$ $att'$ := $att$  $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att'}$). ($\exists$ $ug'$ := $ug$ $\in$ $\effectiveug(u)$. $\Evaluate_{ug}(ug',~c,~s)$ $\wedge$ $val$ $\notin$ $att'$($ug'$) $\wedge$} \State{$\hspace{110mm}$$\exists$ $\mathrm{\langle}$$u$, $e\_{{att'}}$, $vset$$\mathrm{\rangle}$
  %$\langle$ $q$$_{e\_att'}$, $q$$_{e\_att'}$$(u)$ $\rangle$
  $\in$ $q$. $val$ $\in$ $vset$))))}}
  %\State{)}}
  %\State{\textbf{do}}
 % \For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
  %  \State{\textbf{if} $\Evaluate_u(u,~c,~s) = \true$ $\wedge$ $val$ $\notin$ $att$($u$) \textbf{then}}
   % \State{$val$ in rule is not already directly assigned to user $u$ }
   \State{$\hspace{4 mm}$$s$ := $s$ $\ll$ $rule$; \Comment{\texttt{apply rule on state s}}}
   \State{\textbf{switch}}
   \Comment{\texttt{append administrative request to plan}}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddU}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \iffalse
   \State{$\hspace{4 mm}$\textbf{if} $rule$ $\in$ $\mathsf{canAddU}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}
   \State{$\hspace{4 mm}$\textbf{else if} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}
   \State{$\hspace{4 mm}$\textbf{end if}} \fi
  % \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{$\hspace{4 mm}$  Update Direct and Effective attribute assignment of user $u$}
    %\State{$\hspace{4 mm}$$s$ = $t$;}
    %\State{$\hspace{4 mm}$$\mathrm{\langle}$$u, att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$ $\in$ $\eUAAN_s$}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	    % \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	    % \State{$\hspace{8mm}$ $\UAA_t$ == $\UAA_s$
        %     $\backslash$\{$\mathrm{\langle}$$u$, $att$, $att_{s}(u)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
   % att_{s}(u) \cup val$\};}
    %\State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
     %        $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
  %  \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att, val)$);}
    %\State{\textbf{else break;}}
%\EndFor
\iffalse
\LeftComment{\texttt{// Assigning attribute values to effective user groups of user //}}
\For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
%\For{each $att$ $\in$ \ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
    \State{\textbf{if} $\exists$ $ug \in \effectiveug(u)$. $\Evaluate_{ug}(ug,~c,~s) = \true$ $\wedge$ }
    \State{$val$ $\notin$ $att$($ug$) \textbf{then}}
     \State{$\hspace{4 mm}$ $t$ = $s$ $\ll$ $\mathsf{\langle}ar, c, val\mathrm{\rangle}$; \Comment{\texttt{//apply rule on state s//}}}
     \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{to $ug$} \textbf{then}
   % \State{$\hspace{4 mm}$Update Direct attribute assignment of group $ug$ and effective}
   % \State{$\hspace{4 mm}$attributes of user $u$ and transition to state $t$ such that $s$ = $t$;}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	  %   \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	   %  \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
       %      $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $att_{s}(ug)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
  %  att_{s}(ug) \cup val$\};}
   % \State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
    %         $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{else break}}
    \EndFor \fi
    \iffalse
   \For{each $att$ $\in$ ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd_{ug}}_{att}$}
    \State{\textbf{if} $s$ satisfies precondition $c$ $\wedge$
    $(\not\exists$ $\mathrm{\langle}ug, att, sv\mathrm{\rangle}$}
    \State{$\in$ $\UGAAN_s$ such that $val$ $\in$ $sv)$ \textbf{then}}
    \State{$\hspace{4 mm}$  Suppose that $\mathrm{\langle}ug, att, setval\mathrm{\rangle}$ $\in$ $\UGAAN_\gamma$; }
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	     \State{$\hspace{4 mm}$  Go to state $t$ such that}
	     \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
             $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $setval$$\mathrm{\rangle}$\}}
    \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
    setval\cup\{val\}$\};}
    \State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$  $plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{end if}}
    \EndFor
    \fi
 % \State{\textbf{if} $\eUAAN_s$ == $Save$ \textbf{then break;}}
  % \State{$\hspace{0.9 mm}$\textbf{end if}}
\EndWhile
\State{\textbf{if} $s$ $\vdash_{\RPSAME}$ $q$ \textbf{then} \textbf{return}
 $plan$ \textbf{else return false end if} }
 \Comment{\texttt{check if reachability query is satisfied}}
\end{algorithmic}
\end{algorithm*} 

==> Sections/Irrelevant/algo-sup-1+n.tex <==
\begin{algorithm*}[]  \footnotesize
\centering
\caption{Plan Generation for \RPSUPER in [\miniGURANGOP -- $\overline{N}$]}
\label{algo:sup-1+n}
\begin{algorithmic}[1]
\State{\textbf{Input:} problem instance I = $\langle$$\gamma_0$, $q$$\rangle$  \textbf{Output:} $plan$ or false}
\State{$plan$ := $\langle\rangle$;}
\Comment{\texttt{Initialize plan}}
\State{$s$ := $\gamma_0$;}
\Comment{\texttt{Initialize with state s}}
%\State{\textbf{if} $s$ $\vdash_{\RPSUPER}$ $q$ \textbf{then} \textbf{return} $plan$}
% $\langle\rangle$}

%\While{$true$}
%\State{\textbf{Let} $Save$ = $\eUAAN_s$;}
%\LeftComment{\texttt{// Direct attributes assignment to user or user group //}}
\LeftComment{\texttt{Assign all possible attribute values and user groups to the user or user's effective groups}}
\While{($s$ $\nvdash_{\RPSUPER}$ $q$ $\wedge$
\State{((($\exists$ $att'$ := $att$ $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att'}$). ($\Evaluate_u(u,~c,~s)$ $\wedge$ $val$ $\notin$ $att'$($u$)))} \State{ $\lor$} \State{(($\exists$ $att'$ := $att$ $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att'}$). ($\exists$ $ug'$ := $ug$ $\in$ $\effectiveug(u)$. $\Evaluate_{ug}(ug',~c,~s)$ $\wedge$ $val$ $\notin$ $att'$($ug'$)))}
  \State{ $\lor$} \State{(($\exists$ $ug''$ := $ug$ $\in$ \UG $\exists$ $rule$ := $\mathsf{\langle}ar, c, ug''\mathrm{\rangle}$ $\in$ $\Assign$). ($\Evaluate_{u{-}ug}(u,~c,~s)$ $\wedge$ $ug''$ $\notin$ $\directug(u)$))))}}
 % \For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
  %  \State{\textbf{if} $\Evaluate_u(u,~c,~s) = \true$ $\wedge$ $val$ $\notin$ $att$($u$) \textbf{then}}
   % \State{$val$ in rule is not already directly assigned to user $u$ }
   \State{$\hspace{4 mm}$$s$ := $s$ $\ll$ $rule$; \Comment{\texttt{apply rule on state s}}}
   \State{\textbf{switch}}
   \Comment{\texttt{append administrative request to plan}}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddU}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\Assign$:
   \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{assign}(ar, u, ug'')$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \iffalse
   \State{$\hspace{4 mm}$\textbf{if} $rule$ $\in$ $\mathsf{canAddU}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}
   \State{$\hspace{4 mm}$\textbf{else if} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}
   \State{$\hspace{4 mm}$\textbf{else if} $rule$ $\in$ $\Assign$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{assign}(ar, u, ug'')$);}
   \State{$\hspace{4 mm}$\textbf{end if}} \fi
  % \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{$\hspace{4 mm}$  Update Direct and Effective attribute assignment of user $u$}
    %\State{$\hspace{4 mm}$$s$ = $t$;}
    %\State{$\hspace{4 mm}$$\mathrm{\langle}$$u, att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$ $\in$ $\eUAAN_s$}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	    % \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	    % \State{$\hspace{8mm}$ $\UAA_t$ == $\UAA_s$
        %     $\backslash$\{$\mathrm{\langle}$$u$, $att$, $att_{s}(u)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
   % att_{s}(u) \cup val$\};}
    %\State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
     %        $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
  %  \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att, val)$);}
    %\State{\textbf{else break;}}
%\EndFor
\iffalse
\LeftComment{\texttt{// Assigning attribute values to effective user groups of user //}}
\For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
%\For{each $att$ $\in$ \ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
    \State{\textbf{if} $\exists$ $ug \in \effectiveug(u)$. $\Evaluate_{ug}(ug,~c,~s) = \true$ $\wedge$ }
    \State{$val$ $\notin$ $att$($ug$) \textbf{then}}
     \State{$\hspace{4 mm}$ $t$ = $s$ $\ll$ $\mathsf{\langle}ar, c, val\mathrm{\rangle}$; \Comment{\texttt{//apply rule on state s//}}}
     \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{to $ug$} \textbf{then}
   % \State{$\hspace{4 mm}$Update Direct attribute assignment of group $ug$ and effective}
   % \State{$\hspace{4 mm}$attributes of user $u$ and transition to state $t$ such that $s$ = $t$;}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	  %   \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	   %  \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
       %      $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $att_{s}(ug)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
  %  att_{s}(ug) \cup val$\};}
   % \State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
    %         $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{else break}}
    \EndFor \fi
    \iffalse
   \For{each $att$ $\in$ ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd_{ug}}_{att}$}
    \State{\textbf{if} $s$ satisfies precondition $c$ $\wedge$
    $(\not\exists$ $\mathrm{\langle}ug, att, sv\mathrm{\rangle}$}
    \State{$\in$ $\UGAAN_s$ such that $val$ $\in$ $sv)$ \textbf{then}}
    \State{$\hspace{4 mm}$  Suppose that $\mathrm{\langle}ug, att, setval\mathrm{\rangle}$ $\in$ $\UGAAN_\gamma$; }
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	     \State{$\hspace{4 mm}$  Go to state $t$ such that}
	     \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
             $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $setval$$\mathrm{\rangle}$\}}
    \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
    setval\cup\{val\}$\};}
    \State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$  $plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{end if}}
    \EndFor
    \fi
 % \State{\textbf{if} $\eUAAN_s$ == $Save$ \textbf{then break;}}
  % \State{$\hspace{0.9 mm}$\textbf{end if}}
\EndWhile
\State{\textbf{if} $s$ $\vdash_{\RPSUPER}$ $q$ \textbf{then} \textbf{return}
 $plan$ \textbf{else return false end if} }
\Comment{\texttt{check if reachability query is satisfied}}
\end{algorithmic}
\end{algorithm*} 

==> Sections/Irrelevant/algo-sup-1+sr.tex <==
\begin{algorithm*}[] \footnotesize
\centering
\caption{Group Assignment Plan Generation for \RPSUPER in [\miniGURANGOP --$\overline{D}$, \SR]}
\label{algo:sup-1+sr}
\begin{algorithmic}[1]
\State{\textbf{Input:} problem instance I = $\langle$$\gamma_0$, $q$$\rangle$ \textbf{Output:} $plan_{ug}$}
\State{\textbf{if} $\gamma_0$ $\vdash_{\RPSAME}$ $q$ \textbf{then} \textbf{return} $plan_{ug}$  := $\langle\rangle$;}

%\State{$plan_{ug}$ := $\langle \rangle$;}
%\State{\textbf{if} $\exists$ $ug$ $\in$ \UG. $ug$ $\notin$ \directug($u$). $\nexists$ $\mathrm{\langle}ar, c, ug\mathrm{\rangle}$ $\in$ $\Assign(u)$ \textbf{then} }
\State{$G_{ug} := \langle V_{ug}, E_{ug}\rangle$; $V_{ug}$ := \{$ug$ $|$ $\exists$ $ug$ $\in$ \UG. $\exists$ $ug$ $\notin$ $\directug(u)$. $\exists$ $\mathrm{\langle}ar, c, ug\mathrm{\rangle}$ $\in$ $\Assign(u)$ \}; $E_{ug}$ := $\emptyset$;}\Comment{\texttt{Construct a directed graph}}
\For{each pair of nodes ($(ug_1, ug_2) \in V_{ug})$} \State{\textbf{if} (($\exists \mathrm{\langle}ar, c, ug_2\mathrm{\rangle} \in$ $\mathsf{\Assign}$. ``$(ug_1 \in \directug(u))$" is a conjunct in $c$) $\lor$ \State{($\exists \mathrm{\langle}ar, c, ug_1\mathrm{\rangle} \in$
 $\mathsf{\Assign}$. ``$\neg (ug_2 \in \directug(u))$" is a conjunct in $c$))}}
 \State{\textbf{then} $E_{ug}$ := $E_{ug}$ $\cup$ $\{\langle ug_1, ug_2 \rangle\};$ \textbf{end if}} \Comment{\texttt{Add edges}}
\EndFor
\State{\textbf{if} graph $G_{ug}$ has cycles \textbf{then} remove the cyclic paths and $plan_{ug}$ := administrative $\Assign$ request corresponding the topological  sort of $G_{ug}$;}
%\State{\textbf{Pre-Processing}: Before topological sort, \State{ $vset$ is the set of attributes required in query not in $\gamma$.} \State{ Detect in created graph whether there exists a vertex in $vset$ which contains incoming edge from vertex not in $vset$. If yes return false.} \State{ Otherwise, remove all  other vertices not in $vset$. A topological sort of the vertex in $vset$ is a valid plan for the problem. } }
\end{algorithmic}
\end{algorithm*}

 

==> Sections/Irrelevant/algo-sup-1n.tex <==
\begin{algorithm*}[t]  \footnotesize
\centering
\caption{Plan Generation for \RPSUPER in [\miniGURANGO -- $\overline{N}$]}
\label{algo:sup-1n}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\State{\textbf{Input:} problem instance I = $\langle$$\gamma_0$, $q$$\rangle$  \textbf{Output:} $plan$ or false}
\State{$plan$ := $\langle\rangle$;} \Comment{\texttt{Initialize plan}}
\State{$s$ := $\gamma_0$;}
\Comment{\texttt{Initialize with state s}}
%\State{\textbf{if} $s$ $\vdash_{\RPSUPER}$ $q$ \textbf{then} \textbf{return} $plan$;}
% $\langle\rangle$}
%\While{$true$}
%\State{\textbf{Let} $Save$ = $\eUAAN_s$;}
\LeftComment{\texttt{ Assign all possible attribute values to the user or the user's effective groups}}
\While{($s$ $\nvdash_{\RPSUPER}$ $q$ $\wedge$ \State{ ((($\exists$ $att'$ := $att$ $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att'}$). ($\Evaluate_u(u,~c,~s)$ $\wedge$ $val$ $\notin$ $att'$($u$)))}\State{  $\lor$} \State{ (($\exists$ $att'$ := $att$ $\in$ \ATTR $\exists$ $rule$ := $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att'}$). ($\exists$ $ug'$ := $ug$ $\in$ $\effectiveug(u)$. $\Evaluate_{ug}(ug',~c,~s)$ $\wedge$ $val$ $\notin$ $att'$($ug'$))))}}
  %\State{\textbf{do}}
 % \For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
  %  \State{\textbf{if} $\Evaluate_u(u,~c,~s) = \true$ $\wedge$ $val$ $\notin$ $att$($u$) \textbf{then}}
   % \State{$val$ in rule is not already directly assigned to user $u$ }
   \State{$\hspace{4 mm}$$s$ := $s$ $\ll$ $rule$; \Comment{\texttt{apply rule on state s}}}
   \State{\textbf{switch}}
   \Comment{\texttt{append administrative request to plan }}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddU}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$: \State{$\hspace{8 mm}$ $plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \iffalse
   \State{$\hspace{4 mm}$\textbf{if} $rule$ $\in$ $\mathsf{canAddU}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att', val)$);}
   \State{$\hspace{4 mm}$\textbf{else if} $rule$ $\in$ $\mathsf{canAddUG}_{att'}$ \textbf{then}}
   \State{$\hspace{8 mm}$$plan$ := $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug', att', val)$);}
   \State{$\hspace{4 mm}$\textbf{end if}}\fi
  % \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{$\hspace{4 mm}$  Update Direct and Effective attribute assignment of user $u$}
    %\State{$\hspace{4 mm}$$s$ = $t$;}
    %\State{$\hspace{4 mm}$$\mathrm{\langle}$$u, att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$ $\in$ $\eUAAN_s$}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	    % \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	    % \State{$\hspace{8mm}$ $\UAA_t$ == $\UAA_s$
        %     $\backslash$\{$\mathrm{\langle}$$u$, $att$, $att_{s}(u)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
   % att_{s}(u) \cup val$\};}
    %\State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
     %        $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
  %  \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, u, att, val)$);}
    %\State{\textbf{else break;}}
%\EndFor
\iffalse
\LeftComment{\texttt{// Assigning all possible attribute values to effective user groups of user //}}
\For{each attribute $att$ $\in$ \ATTR and rule $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
%\For{each $att$ $\in$ \ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$}
    \State{\textbf{if} $\exists$ $ug \in \effectiveug(u)$. $\Evaluate_{ug}(ug,~c,~s) = \true$ $\wedge$ }
    \State{$val$ $\notin$ $att$($ug$) \textbf{then}}
     \State{$\hspace{4 mm}$ $t$ = $s$ $\ll$ $\mathsf{\langle}ar, c, val\mathrm{\rangle}$; \Comment{\texttt{//apply rule on state s//}}}
     \State{$\hspace{4 mm}$$s$ = $t$;}
   % \State{to $ug$} \textbf{then}
   % \State{$\hspace{4 mm}$Update Direct attribute assignment of group $ug$ and effective}
   % \State{$\hspace{4 mm}$attributes of user $u$ and transition to state $t$ such that $s$ = $t$;}
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	  %   \State{$\hspace{4 mm}$  Go to state $t$ such that}
        % \State{$\hspace{8mm}$ $att_{t}(u)$ = $att_{s}(u)$ $\cup$ $val$ and}
	   %  \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
       %      $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $att_{s}(ug)$$\mathrm{\rangle}$\}}
   % \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
  %  att_{s}(ug) \cup val$\};}
   % \State{$\hspace{8mm}$ $\eUAAN_t$ == $\eUAAN_s$
    %         $\backslash$\{$\mathrm{\langle}$$u$, $att$, $\effu_{s_{\textit{att}}}(u)$$\mathrm{\rangle}$\}}
    %\State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} u, att,
    %\effu_{s_{\textit{att}}}(u) \cup val$\};}
    %\State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$$plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{else break}}
    \EndFor \fi
    \iffalse
   \For{each $att$ $\in$ ATTR and $\mathsf{\langle}ar, c, val\mathrm{\rangle}$ $\in$ $\mathsf{canAdd_{ug}}_{att}$}
    \State{\textbf{if} $s$ satisfies precondition $c$ $\wedge$
    $(\not\exists$ $\mathrm{\langle}ug, att, sv\mathrm{\rangle}$}
    \State{$\in$ $\UGAAN_s$ such that $val$ $\in$ $sv)$ \textbf{then}}
    \State{$\hspace{4 mm}$  Suppose that $\mathrm{\langle}ug, att, setval\mathrm{\rangle}$ $\in$ $\UGAAN_\gamma$; }
    % \State{$\hspace{4 mm}$  $setval^\prime$ = $setval$ $\cup$ \{$val$\}; }
    % \State{$\hspace{4 mm}$  $\UAA_\gamma^\prime$ = $\UAA_\gamma$
             % $\backslash$\{$\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$\}}
	     \State{$\hspace{4 mm}$  Go to state $t$ such that}
	     \State{$\hspace{8mm}$ $\UGAAN_t$ == $\UGAAN_s$
             $\backslash$\{$\mathrm{\langle}$$ug$, $att$, $setval$$\mathrm{\rangle}$\}}
    \State{$\hspace{23 mm}$ $\cup$ $\{\mathrm{\langle} ug, att,
    setval\cup\{val\}$\};}
    \State{$\hspace{4 mm}$ $s$ = $t$;}
    % ^\prime\mathrm{\rangle}\}$;}
    \State{$\hspace{4 mm}$  $plan$ = $plan$.$\mathbf{append}$($\mathsf{add}(ar, ug, att, val)$);}
    \State{\textbf{end if}}
    \EndFor
    \fi
 % \State{\textbf{if} $\eUAAN_s$ == $Save$ \textbf{then break;}}
  % \State{$\hspace{0.9 mm}$\textbf{end if}}
\EndWhile
\State{\textbf{if} $s$ $\vdash_{\RPSUPER}$ $q$ \textbf{then} \textbf{return}
 $plan$ \textbf{else return false end if} }
 \Comment{\texttt{check if reachability query is satisfied}}
\end{algorithmic}
%\end{multicols}
\end{algorithm*} 

==> Sections/Irrelevant/algo-sup-1sr.tex <==
\begin{algorithm*}[t] \footnotesize
\centering
\caption{Plan Generation for \RPSUPER in [\miniGURANGO --$\overline{D}$, \SR]}
\label{algo:sup-1sr}
\begin{algorithmic}[1]
\State{\textbf{Input:} problem instance I = $\langle$$\gamma_0$, $q$$\rangle$
\textbf{Output:} $plan$ or false}
%\State{$toadd$ := $\emptyset$; $cur_{u}$ := $\emptyset$; $ppre_{u}$ := $\emptyset$; $npre_{u}$ := $\emptyset$ ; for each $ug \in \effectiveug(u)$: $cur_{ug}$ := $\emptyset$; $ppre_{ug}$ := $\emptyset$; $npre_{ug}$ := $\emptyset$; $plan$ := $\langle\rangle$;}
%\State{$plan$ := $\langle\rangle$;}%$plan_{ug}$ = $\langle\rangle$;}
\State{\textbf{if} $\gamma_0$ $\vdash_{\RPSUPER}$ $q$ \textbf{then} \textbf{return} $plan$ := $\langle\rangle$;}
\Comment{\texttt{Check initial state}}
\State{$toadd$ := \{($att$, $val$) $|$ $att$ $\in$ \ATTR, $\mathrm{\langle}$$u$, $e\_{{att}}$, $vset$$\mathrm{\rangle}$ $\in$ $q$, $val$ $\in$ $vset$\}}\Comment{\texttt{Values required in query}}
\State{$cur_{u}$ := \{($att$, $val$) $|$ $att$ $\in$ \ATTR, $val$ $\in$ $att(u)$\}}\Comment{\texttt{Current values of user}}
\State{\textbf{for} each $ug$ $\in$ $\effectiveug($u$)$ \textbf{do} $cur_{ug}$ := \{($att$, $val$) $|$ $att$ $\in$ \ATTR, $val$ $\in$ $att(ug)$\} \textbf{end for}}\Comment{\texttt{Current values of user's effective groups}}
%\State{ $\forall$ $\mathrm{\langle}$u, att, vset$\mathrm{\rangle}$ $\in$ $\UAA_\gamma$. $\forall$
%val $\in$ vset.  }
%\State{$\hspace{4 mm}$ $cur^\prime_u$ = $cur$ $\cup$ \{(att, val)\};}
%\LeftComment{\texttt{// Find current direct attributes of user and all its effective user groups in state $\gamma$ //}}
\iffalse
\While{(($\exists$ $att'$ := $att$ $\in$ $\ATTR$ $\exists$ $val'$ := $val$ $\in$ $att'(u)$ $\wedge$ $(att', val')$ $\notin$ $cur_{u}$) \State{ $\lor$} \State{ ($\exists$ $ug'$ := $ug$ $\in$ \effectiveug($u$) $\exists$ $att''$ := $att$ $\in$ $\ATTR$ $\exists$ $val''$ := $val$ $\in$ $att''(ug')$ $\wedge$ $(att'', val'')$ $\notin$ $cur_{ug'}$)} \State{ $\lor$} \State{ ($\exists$ $q$$_{e\_att'''}$($u$) $\in$ $q$ $\exists$ $val'''$ $\in$ $q$$_{e\_att'''}$($u$) $\wedge$ $(att''', val''')$ $\notin$ $toadd$))}}
\State{\textbf{switch}}
   %\Comment{\texttt{append administrative request to plan}}
   \State{$\hspace{4 mm}$\textbf{case} $(att', val')$ $\notin$ $cur_{u}$: \State{$\hspace{8 mm}$ $cur_{u}$ := $cur_{u}$ $\cup$ \{$(att', val')$\};}}\Comment{\texttt{Current values of user}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $(att'', val'')$ $\notin$ $cur_{ug'}$: \State{$\hspace{8 mm}$ $cur_{ug'}$ := $cur_{ug'}$ $\cup$ \{$(att'', val'')$\};}}\Comment{\texttt{Current values of effective user groups}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} $(att''', val''')$ $\notin$ $toadd$:
   \State{$\hspace{8 mm}$ $toadd$ := $toadd$ $\cup$ \{$(att''', val''')$\};}}\Comment{\texttt{Values required in query}}
   \State{$\hspace{4 mm}$\textbf{break};}
\EndWhile \fi
\iffalse
\While{($\exists$ $att'$ := $att$ $\in$ $\ATTR$ $\exists$ $val'$ := $val$ $\in$ $att'(u)$)}
\State{$\hspace{4 mm}$ $cur_{u}$ := $cur_{u}$ $\cup$ \{$(att, val)$\};}
\Comment{\texttt{Current values of user}}
\EndWhile
\While{($\exists$ $ug'$ := $ug$ $\in$ \effectiveug($u$) $\exists$ $att''$ := $att$ $\in$ $\ATTR$ $\exists$ $val''$ := $val$ $\in$ $att''(ug')$)}
\State{$\hspace{4 mm}$ $cur_{ug}$ := $cur_{ug}$ $\cup$ \{$(att, val)$\};}
\Comment{\texttt{Current values of effective user groups}}
\EndWhile
\fi
\iffalse
\While{($\exists$ $att$ $\in$ $\ATTR$ $\exists$ $val$ $\in$ $att(u)$ $\wedge$ $(att, val)$ $\notin$ $cur_{u}$)}
\State{$\hspace{4 mm}$ $cur_{u}$ := $cur_{u}$ $\cup$ \{$(att, val)$\};}
\Comment{\texttt{Current values of user}}
\EndWhile
\While{($\exists$ $ug$ $\in$ \effectiveug($u$) $\exists$ $att$ $\in$ $\ATTR$ $\exists$ $val$ $\in$ $att(ug)$ $\wedge$ $(att, val)$ $\notin$ $cur_{ug}$)}
\State{$\hspace{4 mm}$ $cur_{ug}$ := $cur_{ug}$ $\cup$ \{$(att, val)$\};}
\Comment{\texttt{Current values of effective user groups}}
\EndWhile
%\State{$\forall$ $att$ $\in$ $\ATTR$  $\forall$ $val$ $\in$ $att(u)$}

%\State{$\hspace{4 mm}$ $cur_{u}$ = $cur_{u}$ $\cup$ \{$(att, val)$\};}
%\Comment{\texttt{Current values of user}}
%\EndFor
%\State{for all $ug \in \effectiveug(u)$:}
%\State{$\forall$ $ug$ $\in$ \effectiveug($u$) $\forall$ $att$ $\in$ $\ATTR$ $\forall$ $val$ $\in$ $att(ug)$}
%\State{for each $att$ $\in$ $\ATTR$ and for each $val$ $\in$ $att(u)$:}
%\State{$\hspace{4 mm}$ $cur_{ug}$ = $cur_{ug}$ $\cup$ \{$(att, val)$\};}
%\Comment{\texttt{Current values of effective user groups}}
%\EndFor
%\LeftComment{\texttt{// Find all values required to satisfy query //}}
\While{($\exists$ \qe($u$) $\in$ $q$ $\exists$ $val$ $\in$ \qe($u$) $\wedge$ $(att, val)$ $\notin$ $toadd$)}
\State{$\hspace{4 mm}$ $toadd$ := $toadd$ $\cup$ \{$(att, val)$\};}
\Comment{\texttt{Values required in query}}
\EndWhile \fi
%\State{$\forall$ \qe($u$) $\in$ $q$ $\forall$ $val$ $\in$ \qe($u$)}
%\State{$\hspace{4 mm}$ $toadd^\prime_e$ = $toadd^\prime_e$ $\cup$ \{$(att, val)$\};}
%\Comment{\texttt{Values required in query}}
%\State{\textbf{Repeat}:}
%\EndFor
%\LeftComment{\texttt{Find positive precondition values required by the user and the user's effective groups to satisfy query}}
\iffalse
\State{$\forall$ $(att, val)$ $\in$ $toadd^\prime_e$ }
\State{$\hspace{2 mm}$\textbf{Repeat}:}
\State{ $\hspace{4 mm}$ $ppre_u$ = \{$(att_1, val_1)_{u}$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$ such}
\State{$\hspace{10 mm}$ that $val_1\in att_1(u)$ is a conjunct in $c$\};}
\State{ $\hspace{4 mm}$ $ppre_u$ = $ppre_u$ $\cup$ \{$(att_1, val_1)_{u}$\}$\backslash$$cur_{u}$;}
\State{$\hspace{2 mm}$\textbf{Until $ppre_u$ does not change}:}
%\State{\textbf{Repeat}:}
\State{$\hspace{2 mm}$\textbf{Repeat}:}
\State{$\hspace{4 mm}$$\forall$ $ug \in \effectiveug(u)$:}
\State{ $\hspace{4 mm}$ $ppre_{ug}$ = \{$(att_1, val_1)_{ug}$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$ such}
\State{$\hspace{10 mm}$ that $val_1\in att_1(ug)$ is a conjunct in $c$\};}
\State{ $\hspace{4 mm}$ $ppre_{ug}$ = $ppre_{ug}$ $\cup$ \{$(att_1, val_1)_{ug}$\}$\backslash$$cur_{ug}$;}
\State{$\hspace{2 mm}$\textbf{Until $ppre_{ug}$ does not change}:}

\State{$\hspace{0 mm}$\textbf{Repeat}:}
\State{$\hspace{0 mm}$$\forall$ $(att, val)$ $\in$ $toadd^\prime_e$ $\cup$ $ppre_u$}
\State{ $\hspace{2 mm}$ $ppre_u$ = \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$ such that $val_1\in att_1(u)$ is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
\State{ $\hspace{2 mm}$ $ppre_u$ = $ppre_u$ $\cup$ \{$(att_1, val_1)$\}$\backslash$$cur_{u}$;}
\State{$\hspace{0 mm}$\textbf{Until $ppre_u$ does not change}:}\fi
\State{$ppre_{u}$ := $\emptyset$; \textbf{for} each $ug \in \effectiveug(u)$ \textbf{do} $ppre_{ug}$ := $\emptyset$; \textbf{end for}}
%\State{$ppre_{u}$ := $\emptyset$; $npre_{u}$ := $\emptyset$;}
%\State{\textbf{for} each $ug \in \effectiveug(u)$ \textbf{do} $ppre_{ug}$ := $\emptyset$; $npre_{ug}$ := $\emptyset$ \textbf{end for}}
%\For{each $ug \in \effectiveug(u)$} \State{$ppre_{ug}$ := $\emptyset$; $npre_{ug}$ := $\emptyset$}
%\EndFor
\For{(each $(att, val)$ $\in$ $toadd$ $\cup$ $ppre_u$)}
\Comment{\texttt{Positive precondition values for user}}
\State{$\hspace{2 mm}$ $ppre'_u$ := \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$. ``$val_1\in att_1(u)$" is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
%\State{$\hspace{2 mm}$ $ppre''_u$ := $ppre_u$ $\cup$ $ppre'_u$ $\backslash$ $cur_{u}$;}
\State{$\hspace{2 mm}$ $ppre_u$ := ( $ppre_u$ $\cup$ ($ppre'_u$ $\backslash$ $ppre_u$ )) $\backslash$ $cur_{u}$;}
\EndFor
\For{(each $ug \in \effectiveug(u)$)}
\Comment{\texttt{Positive precondition values for effective groups}}
\For{(each $(att, val)$ $\in$ $toadd$ $\cup$ $ppre_{ug}$)}
\State{$ppre'_{ug}$ := \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$. ``$val_1\in att_1(ug)$" is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
%\State{$\hspace{2 mm}$ $ppre''_{ug}$ := $ppre_{ug}$ $\cup$ $ppre'_{ug}$ $\backslash$ $cur_{ug}$;}
\State{$ppre_{ug}$ := ( $ppre_{ug}$ $\cup$  ($ppre'_{ug}$ $\backslash$ $ppre_{ug}$)) $\backslash$ $cur_{ug}$;}
\EndFor
\EndFor
\iffalse
\While{($\exists$ $(att, val)$ $\in$ $toadd$ $\cup$ $ppre_u$)}
\Comment{\texttt{Positive precondition values for user}}
\State{$\hspace{2 mm}$ $ppre'_u$ := \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$. ``$val_1\in att_1(u)$" is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
%\State{$\hspace{2 mm}$ $ppre''_u$ := $ppre_u$ $\cup$ $ppre'_u$ $\backslash$ $cur_{u}$;}
\State{$\hspace{2 mm}$ \textbf{if} $ppre'_u$ == $ppre_u$ \textbf{then break}; \textbf{else} $ppre_u$ := 
( $ppre_u$ $\cup$ $ppre'_u$ ) $\backslash$ $cur_{u}$;}
\EndWhile
\While{($\exists$ $ug \in \effectiveug(u)$ $\exists$ $(att, val)$ $\in$ $toadd$ $\cup$ $ppre_{ug}$)}
\Comment{\texttt{Positive precondition values for effective groups}}
\State{$\hspace{2 mm}$ $ppre'_{ug}$ := \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$. ``$val_1\in att_1(ug)$" is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
%\State{$\hspace{2 mm}$ $ppre''_{ug}$ := $ppre_{ug}$ $\cup$ $ppre'_{ug}$ $\backslash$ $cur_{ug}$;}
\State{$\hspace{2 mm}$ \textbf{if} $ppre'_{ug}$ == $ppre_{ug}$ \textbf{then break}; \textbf{else} $ppre_{ug}$ := ( $ppre_{ug}$ $\cup$  $ppre'_{ug}$ ) $\backslash$ $cur_{ug}$;}
\EndWhile \fi
%\State{\textbf{Repeat}:}
\iffalse
\State{$\hspace{0 mm}$\textbf{Repeat}:}
\State{$\hspace{0 mm}$ $\forall$ $ug \in \effectiveug(u)$ $\forall$ $(att, val)$ $\in$ $toadd^\prime_e$ $\cup$ $ppre_{ug}$}
%\State{$\hspace{4 mm}$$\forall$ $ug \in \effectiveug(u)$:}
\State{ $\hspace{2 mm}$ $ppre_{ug}$ = \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$ such that $val_1\in att_1(ug)$ is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
\State{ $\hspace{2 mm}$ $ppre_{ug}$ = $ppre_{ug}$ $\cup$ \{$(att_1, val_1)$\}$\backslash$$cur_{ug}$;}
\State{$\hspace{0 mm}$\textbf{Until $ppre_{ug}$ does not change}:} \fi
%\EndFor
%\State{\textbf{or else check for all $ ug \in \effectiveug(u)$}:}
%\State{ $\hspace{4 mm}$ $ppre$ = $ppre$ $\cup$ \{$(att_1, val_1)_{ug}$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
%\mathrm{\rangle}$
%$\in$ $\mathsf{canAdd}_{att}$ such}
%\State{$\hspace{10 mm}$ that $val_1\in att_1(ug)$, is a conjunct in $c$\};}
%\State{ $\hspace{4 mm}$ $toadd^\prime_e$ = $toadd^\prime_e$ $\cup$ $ppre$
% $\backslash$ $cur^\prime_{e}$;}
%\State{\textbf{Until $toadd^\prime_e$ does not change}}
%\State{\textbf{if} $\exists$ $(att, val)$ $\in$ $toadd^\prime_e$ such that $\nexists$ $\mathrm{\langle}ar,c, val
%\mathrm{\rangle}\in \mathsf{canAdd}_{att}$ }
%\State{\textbf{then return false end if}}
\LeftComment{\texttt{ Check if rules exists for values required }}
\State{\textbf{if} (($\exists(att, val)$ $\in$ $toadd$ $\cup$ $ppre_u$ $\cup$ $(\bigcup\limits_{ug \; \in\; \effectiveug(u)}ppre_{ug})$  $\backslash$ ($cur_u$ $\cup$ $(\bigcup\limits_{ug \; \in\; \effectiveug(u)} cur_{ug})))$. $\nexists$ $\mathrm{\langle}ar, c, val \mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$ $\cup$ $\mathsf{canAddUG}_{att}$)\textbf{then return} false;}
%\State{\textbf{if} (($\exists(att, val)$ $\in$ $toadd$ $\cup$ $ppre_u$ $\backslash$ $cur_u$. $\nexists$ $\mathrm{\langle}ar, c, val \mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$) $\wedge$} \State{$\hspace{2 mm}$ ($\forall$ $ug$ $\in$ \effectiveug($u$) $\exists(att, val)$ $\in$ $toadd$ $\cup$ $ppre_{ug}$ $\backslash$ $cur_{ug}$. $\nexists$ $\mathrm{\langle}ar, c, val \mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$)) \textbf{then return} false;}
%\State{\textbf{else return false}; \textbf{end if}}
%\iffalse
\LeftComment{\texttt{Find negation values in rules required to add values for the user and its effective groups}}
\State{$npre_u$ := \{($att_1$, $val_1$) $|$ $\exists$ $(att, val)$ $\in$ ( $toadd$ $\cup$ $ppre_u$ ) $\backslash$ $cur_u$ . $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$. ``$\neg (val_1\in att_1(u))$" is a conjunct in $c$\}}%\Comment{\texttt{negation for user}}
\State{\textbf{for} each $ug \in \effectiveug(u)$ \textbf{do} $npre_{ug}$ := \{($att_1$, $val_1$) $|$ $\exists$ $(att, val)$ $\in$ ($toadd$ $\cup$ $ppre_{ug}$) $\backslash$ $cur_{ug}$ . $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$. ``$\neg (val_1\in att_1(ug))$" is a conjunct in $c$\} \textbf{end for}}%\Comment{\texttt{negation for effective groups}}
%\fi
\iffalse
\While{($\exists$ $(att, val)$ $\in$ $ppre_u$ $\cup$ $toadd$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$)}
\State{ $\hspace{4 mm}$ $npre_u$ := $npre_u$ $\cup$ \{$(att_1, val_1)$ $|$ $\neg (val_1\in att_1(u))$ is in $c$\}}
\Comment{\texttt{negation values in rules for user}}
\EndWhile
\While{($\exists$ $ug \in \effectiveug(u)$ $\exists$ $(att, val)$ $\in$ $ppre_{ug}$ $\cup$ $toadd$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$)}
\State{ $\hspace{4 mm}$ $npre_{ug}$ := $npre_{ug}$ $\cup$ \{$(att_1, val_1)$ $|$ $\neg (val_1\in att_1(ug))$ is in $c$\}}
\Comment{\texttt{negation values for effective groups}}
\EndWhile \fi
\iffalse
\State{$\forall$ $(att, val)$ $\in$ $ppre_u$ $\cup$ $toadd^\prime_e$ }
%\State{\textbf{Repeat}:}
\State{ $\hspace{4 mm}$ $npre_u$ = \{$(att_1, val_1)$ $|$ $\exists$ $\mathrm{\langle}ar, c, val
\mathrm{\rangle}$ $\in$ $\mathsf{canAddU}_{att}$ such that $\neg (val_1\in att_1(u))$ is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
\State{ $\hspace{4 mm}$ $npre_u$ = $npre_u$ $\cup$ \{$(att_1, val_1)$\};}
%\State{\textbf{Until $npre_u$ does not change}:}
%\State{\textbf{Repeat}:}
%\State{\textbf{Repeat}:}
\State{$\forall$ $ug \in \effectiveug(u)$ $\forall$ $(att, val)$ $\in$ $ppre_{ug}$ $\cup$ $toadd^\prime_e$ }
\State{ $\hspace{4 mm}$ $npre_{ug}$ =\{$(att_1, val_1)$$|$ $\exists$ $\mathrm{\langle}ar, c, val \mathrm{\rangle}$ $\in$ $\mathsf{canAddUG}_{att}$ such that $\neg (val_1\in att_1(ug))$ is a conjunct in $c$\};}
%\State{$\hspace{10 mm}$ that }
\State{ $\hspace{4 mm}$ $npre_{ug}$ = $npre_{ug}$ $\cup$ \{$(att_1, val_1)$\};}
%\State{\textbf{Until $npre_{ug}$ does not change}:}
%\EndFor
\fi
%\LeftComment{\texttt{If certain values in negation conjuncts are present in current values of user and all its effective user groups then return false}}
\State{\textbf{if} ($npre_u$ $\cap$ $cur_{u}$ $\neq$ $\emptyset$) $\lor$ ($\forall$ $ug$ $\in$ \effectiveug($u$). $npre_{ug}$ $\cap$ $cur_{ug}$ $\neq$ $\emptyset$) \textbf{then return} false;}
\Comment{\texttt{Negation in current values}}
%\State{$\forall$ $(att, val)$ $\in$ $toadd^\prime_e$}
%\State{$\hspace{4 mm}$$npre$ = $npre$ $\cup$ \{$(att_1, val_1)$ $|$ $\exists$ $
%\mathrm{\langle}ar, c, val\mathrm{\rangle}$
%$\in$ $\mathsf{canAdd}_{att}$ such}
%\State{$\hspace{10 mm}$that $\neg (val_1\in att_1(u))$ or for $ ug \in \effectiveug(u)$ such}
 %\State{{$\hspace{10 mm}$that $\neg (val_1\in att_1(ug))$  is a conjunct in $c$\};}}
%\State{\textbf{if} $npre$ $\cap$ $cur^\prime_{e}$ != $\emptyset$ \textbf{then return false end if}}
%\LeftComment{\texttt{Construct directed graph for user and effective user groups}}
%\State{$G := \langle V, E\rangle$; $V$ := $toadd$ $\cup$ $ppre_{u}$ $\cup$ \{$ppre_{ug}$ $|$ $ug$ $\in$ \effectiveug(u)\}; $E$ := $\emptyset$;}\Comment{\texttt{Construct a directed graph}}
\State{$G := \langle V, E\rangle$; $V$ := $toadd$ $\cup$ $ppre_{u}$ $\cup$ $(\bigcup\limits_{ug \; \in\; \effectiveug(u)}ppre_{ug})$ $\backslash$ ($cur_u$ $\cup$ $(\bigcup\limits_{ug \; \in\; \effectiveug(u)} cur_{ug}))$; $E$ := $\emptyset$;}\Comment{\texttt{Construct a directed graph}}


%\State{$V$ = $toadd$ $\cup$ $ppre_{u}$ $\cup$ \{$ppre_{ug}$ $|$ $ug$ $\in$ \effectiveug(u)\}; $E$ = $\emptyset$;}
%\State{V1 = $toadd^\prime_e$ $\cup$ $ppre_{u}$; V2 = $toadd^\prime_e$ $\cup$  $ppre_{ug}$; $V$ = V1 $\cup$ V2; $E$ = $\emptyset$;}
%\State{$\hspace{4 mm}$ V2 = $toadd^\prime_e$ $\cup$  $ppre_{ug}$;}
\For{each pair of nodes ($(att_1, val_1),(att_2, val_2)$) $\in$ $V$} \State{\textbf{if} ((($\exists \mathrm{\langle}ar, c, val_2\mathrm{\rangle} \in$ $\mathsf{canAddU}_{att_2}$. ``$(val_1 \in att_1(u))$" is a conjunct in $c$) $\lor$ \State{($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in$
 $\mathsf{canAddU}_{att_1}$. ``$\neg (val_2 \in att_2(u))$" is a conjunct in $c$))}} \State{ $\lor$} \State{(($\exists$ $ug \in \effectiveug(u)$). (($\exists \mathrm{\langle}ar, c, val_2\mathrm{\rangle} \in \mathsf{canAddUG}_{att_2}$. ``$(val_1 \in att_1(ug))$" is a conjunct in $c$) $\lor$ \State{($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in$ $\mathsf{canAddUG}_{att_1}$. ``$\neg (val_2 \in att_2(ug))$" is a conjunct in $c$))))}}
%\State{\textbf{if} ($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in \mathsf{canAdd}_{att}
%\mathrm{ ~such~that}~val \in att(u)$ is a}
%\State{conjunct in c) $\vee$ ($\exists
%\mathrm{\langle}ar, c, val\mathrm{\rangle} \in \mathsf{canAdd}_{att}$ such that $\neg (val_1 \in
%att_1(u))$ is a }
%\State{conjunct in c)}
%\State{\textbf{if} ($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in \mathsf{canAddU}_{att} \mathrm{ ~such~that}~val \in att(u)$ is a}
%\State{ $\hspace{4 mm}$  $ ug \in \effectiveug(u)$ such that $val_1\in att_1(ug)$ is a conjunct in c) }
%\State{$\hspace{4 mm}$ conjunct in c $\vee$ ($\exists \mathrm{\langle}ar, c, val\mathrm{\rangle} \in \mathsf{canAdd}_{att}$ such that}
%\State{ $\hspace{4 mm}$for $ug \in \effectiveug(u)$ such that $\neg(val_1\in att_1(ug))$}
%\State{$\neg (val_1 \in$ $att_1(u))$ is a conjunct in c)}
\State{\textbf{then} $E := E$ $\cup$ \{$\langle(att_1, val_1),(att_2, val_2)\rangle$\}; \textbf{end if}}\Comment{\texttt{Add edges to the graph}}
\EndFor
\iffalse
\While{$\exists$ $ug \in \effectiveug(u)$ $\exists$ ($(att, val),(att_1, val_1)$) $\in$ V2}
%\For{each pair of nodes ($(att, val),(att_1, val_1)$) $\in$ V2}
%\State{\textbf{if} ($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in \mathsf{canAdd}_{att}
%\mathrm{ ~such~that}~val \in att(u)$ is a}
%\State{conjunct in c) $\vee$ ($\exists
%\mathrm{\langle}ar, c, val\mathrm{\rangle} \in \mathsf{canAdd}_{att}$ such that $\neg (val_1 \in
%att_1(u))$ is a }
%\State{conjunct in c)}
\State{\textbf{if} ($\exists \mathrm{\langle}ar, c, val_1\mathrm{\rangle} \in \mathsf{canAdd}_{att}
\mathrm{ ~such~that}~val \in att(ug)$}
\State{ $\hspace{4 mm}$ is conjunct in c) $\vee$ ($\exists
\mathrm{\langle}ar, c, val\mathrm{\rangle} \in \mathsf{canAdd}_{att}$ such that}
\State{$\hspace{4 mm}$ $\neg (val_1\in
att_1(ug))$ is a conjunct in c)}
%\State{ $\hspace{4 mm}$ or for $ug \in \effectiveug(u)$ such that $\neg(val_1\in att_1(ug))$}
%\State{ $\hspace{4 mm}$ }
\State{\textbf{then} E$^\prime$ = E $\cup$ \{$\langle(att, val),(att_1, val_1)\rangle$\};
\textbf{end if}}
\EndWhile
%\EndWhile

%\State{Remove all paths with cycles}
\State{G$_u$= $\mathrm{\langle} V_u, E_u \mathrm{\rangle}$;} \Comment{\texttt{subgraph for u}}
\State{\textbf{for} each $ug \in \effectiveug(u)$ \textbf{do} G$_{ug}$= $\mathrm{\langle} V_{ug}, E_{ug} \mathrm{\rangle}$ \textbf{end for};} \Comment{\texttt{subgraph for effective groups}}
\While{($\exists$ ($att$, $val$) $\in$ $toadd$ $\wedge$ ((($att$, $val$) $\in$ $V_u$) $\lor$ ($\exists$ $ug \in \effectiveug(u)$ ($att$, $val$) $\in$ $V_{ug}$)))}
\State{\textbf{switch}}
  % \Comment{\texttt{append administrative request to plan }}
   \State{$\hspace{4 mm}$\textbf{case} G$_u$ has a cycle: \State{$\hspace{8 mm}$ $V_u =: V_u \backslash (att, val); $} \State{$\hspace{8 mm}$ $E:= E$ $\backslash$ \{$(att_1,val_1), (att, val) | (att_1,val_1) \in  V_u$ \};}}
   \State{$\hspace{4 mm}$\textbf{break};}
   \State{$\hspace{4 mm}$\textbf{case} G$_{ug}$ has a cycle: \State{$\hspace{8 mm}$ $V_{ug} =: V_{ug} \backslash (att, val); $} \State{$\hspace{8 mm}$ $E:= E$ $\backslash$ \{$(att_1,val_1), (att, val) | (att_1,val_1) \in  V_{ug}$ \};}}
   \State{$\hspace{4 mm}$\textbf{break};}
\EndWhile \fi
\iffalse
\For{each ($att$, $val$) $\in$ $toadd$}
\State{Let subgraph for $u$, G$_u$= $\mathrm{\langle} V_u, E_u \mathrm{\rangle}$ such that ($att$, $val$) $\in$ V$_u$}
\State{$\hspace{4 mm}$ \textbf{if} G$_u$ has a cycle \textbf{then} $E_u:= E_u$ $\backslash$ \{$(att_1,val_1), (att, val) | (att_1,val_1) \in  V_u$ \}  }
\EndFor

\State{\textbf{if} $\exists$ ($att$, $val$) $\in$ $toadd$ $\forall ug \in \effectiveug(u)$. ($att$, $val$) $\notin$ $V_u \cup V_{ug}$ \textbf{then return} false. } \fi
\iffalse
\State{\textbf{for} each ($att$, $val$) $\in$ $toadd$ \textbf{do}  detect in created graph whether there exists cycle in subgraph having incoming edge to ($att$, $val$)}
\State{\textbf{for} each ($att$, $val$) $\in$ $toadd$ \textbf{do} find if subgraphs for $u$ and for each $ug$ $\in$ $\effectiveug(u)$ has cycle.}

\State{$\hspace{4 mm}$\textbf{if} all subgraphs have cycle \textbf{then return} false \textbf{else} remove all incoming edges to ($att$, $val$) from the subgraph.}
\fi
%\State{$\hspace{4 mm}$\textbf{if} all subgraphs have cycle \textbf{then return} false \textbf{else} ignore the subgraph with cycle and incoming edges of the subgraph to ($att$, $val$).}
%\State{else ignore the subgraph with cycle and incoming edges of the subgraph to ($att$, $val$).}
\State{\textbf{if} graph G has a cycle \textbf{then return} false \textbf{else return} $plan$ := administrative requests corresponding to the topological sort of G;}
%\State{\textbf{if} graph G has a cycle \textbf{then return} false \textbf{else return} $plan$ := topological sort of G}

%\State{\textbf{if} remaining graph has a cycle \textbf{then return} false \textbf{else return} $plan$ := topological sort of graph}
\iffalse
%\State{ find all incoming paths with cycles. Remove all edges and vertices along the path. If no incoming edge, return false.}}}
\State{$plan$ = Topological ordering on remaining graph}
%\State{/*Because of \SR\xspace restriction, it is easy to retrieve administrative role for each
%action in $plan$ */}
\State{\textbf{if} topological ordering is successful \textbf{then return} $plan$ else return false \textbf{end if}} \fi
\end{algorithmic}
\end{algorithm*} 

==> Sections/Irrelevant/sa-1+-n.tex <==
%\smallskip
In \RPSAME for $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ scheme, the values to be added should be present in the query. Also, if the assignment of new group to user results in extra values not in query, the group assignment is not allowed.
\iffalse
In \RPSAME for $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ scheme, we made some minor changes in Algorithm \ref{algo:sup-1+n} by checking the attribute value or user group to be added with the set of values required in query $q$. If the value is not present in the query or the assignment of a new user group results in values not in query, we will not add corresponding action into the plan.
\fi% This extra condition is checked for user and all the effective user-groups of the user.

\begin{thm}\label{}
Reachability query type \RPSAME for scheme $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ is P.
\end{thm}
\begin{proof}
Algorithm \ref{algo:sa-1+n} describes the polynomial time algorithm.
\end{proof}


\noindent
\iffalse
\textbf{Correctness:} The only change with respect to the Algorithm \ref{alg:algo-su-1+-n} is the assignment of new user groups. Hence, the proof of correctness can be very well comprehended. % The algorithm involves a minor change of adding more effective user-groups to the user and giving more values as compared to algorithm \ref{alg:algo-sa-1-n}.
\fi
\noindent
\textbf{Complexity:} With more administrative rules for assigning new user-groups, the added complexity is $\mathcal{O}$($|\mathsf{\Assign}|$ $\times$ $|\UG|$) since with every traverse in the first for loop, only one user group is added. Thus, the total complexity is $\mathcal{O}$($|\mathsf{\Assign}|$ $\times$ $|\UG|$ + ($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ ( $|\mathsf{\canA_{att}}|$ + $|\mathsf{\canAUG_{att}}|$ $\times$ $|\effectiveug|$ )) which is polynomial.

%The complexity is similar to Algorithm \ref{algo:sup-1+n}. 

==> Sections/Irrelevant/sa-1+-sr.tex <==
\RPSAME for $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ also checks if the group to be added do not have more attributes than required in the query. Algorithm \ref{algo:sa-1+sr} creates the plan $plan_{ug}$, where a directed graph is created with vertices as groups not already in user with no extra attributes than required in query and edges are directed based on dependence. Once new effective groups are calculated, the algorithm works similar to Algorithm \ref{algo:sa-1sr}.

%We will add pre-processing step similar to \RPSUPER for $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ scheme with extra check to find the effective groups of the user.

\begin{thm}\label{}
Reachability query type \RPSAME for scheme $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ is P.
\end{thm}
\begin{proof}
%Algorithm \ref{alg:algo-sa-1+-sr} describes the polynomial time algorithm.
%Same as above just with the change in topological sort as in previous Theorem 4.
Algorithm \ref{algo:sa-1+sr} describes algorithm for group assignment plan followed by reachability plan generated by Algorithm \ref{algo:sa-1sr}.
%Algorithm \ref{algo:sa-1+sr} describes the polynomial time algorithm.
\end{proof}
\iffalse
\textbf{Correctness:} The only change required from Algorithm \ref{alg:algo-su-1+-sr} is the removal of vertices not in $valset$, before creating topological sort. If no edge reaches all the values in $toadd^\prime_e$, the query is not satisfiable.
\fi
\smallskip
\noindent
\textbf{Complexity:}  The added step to create a separate graph for group assignment plan will have complexity of $\mathcal{O}$($|\UG|$ $\times$ $|\mathsf{\Assign}|$). Total complexity for \RPSAME for $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ is $\mathcal{O}$($|\UG|$ $\times$ $|\mathsf{\Assign}|$ + (($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ ($|\mathsf{\canA_{att}}|$ + $|\canAUG_{att}|$ $\times$ $|\effectiveug|$))).

%\clearpage 

==> Sections/Irrelevant/sa-1-n.tex <==
\smallskip
In \RPSAME for $\mathrm{[\miniGURANGO{-}\overline{N}]}$ scheme, we are looking for a state where the reachability query is strictly satisfied, i.e the values for attributes in the state should be exactly the same with no extra values. Therefore, we made some minor changes in Algorithm \ref{algo:sup-1n} by checking the value to be added with the set of values required in query $q$. If the value is not present in the query, we will not add the value to user or its effective groups. Also we check if the current state do not have more values than the query, as the user will never satisfy the query (since delete rules are not required).
%This extra condition is checked for user and all the effective user-groups of the user.
\begin{thm}\label{}
Reachability query type \RPSAME for scheme $\mathrm{[\miniGURANGO{-}\overline{N}]}$ is P.
\end{thm}
\begin{proof}
%Algorithm \ref{algo:sa-1n} describes the polynomial time algorithm.
Detailed algorithm is discussed in appendix.
\end{proof}
\noindent
\iffalse
\textbf{Correctness:} The only change in Algorithm \ref{alg:algo-sa-1-n} is in the conditions checked for adding attribute values. Therefore, if some values, outside the values in query $q$, are required in pre-condition to add new values, the algorithm will not allow them and will return false.
%Therefore, if some values are required to add new values, the precondition will restrict the addition of new values and may return false, resulting in no $plan$.
\fi
\smallskip
\noindent
\textbf{Complexity:} The algorithm adds an extra check to search values in query before adding to the user or groups. This search is a polynomial time operation and therefore the algorithm is polynomial time with the same complexity as Algorithm \ref{algo:sup-1n}.
% $\mathcal{O}$($|vset|$ $\times$ $\sum_{att \in \ATTR}$$|\SCOPE_{att}|$).


==> Sections/Irrelevant/sa-1-sr.tex <==

%\smallskip
 The \RPSAME for $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ scheme can be solved by extending the algorithm for \RPSUPER for $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ scheme. Since this scheme requires exact query to be satisfied, some pre-processing is done before creating a topological sort. Assuming $valset$ as the set of attribute values in query $q$ not in state $\gamma_0$. If in the created graph the edges incoming to the attribute value pair in set $valset$ are from the pair not in $valset$, the algorithm returns false. Otherwise, remove all the vertices not in $valset$ and there corresponding edges. Topological sort of the modified graph will provide the path to satisfy the query.
 %The new topological sort will give the path after ignoring all user and user-groups which require subset of values.

 % The directed graph will have multiple paths for each attribute value pair in $toadd^\prime_e$.  If in created directed graph all the edges reaching to same attribute-value have incoming edges from vertices not in $valset$ return false, since no path would then exist.

\begin{thm}\label{}
Reachability query type \RPSAME for scheme $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ is P.
\end{thm}
\begin{proof}
Algorithm \ref{algo:sa-1sr} describes the polynomial time algorithm.
\end{proof}
\iffalse
\textbf{Correctness:} The only change required from Algorithm \ref{alg:sup-1sr} is the removal of vertices not in $valset$, before creating topological sort. If no edge reaches all the values in $toadd^\prime_e$, the query is not satisfiable.
\fi
\smallskip
\noindent
\textbf{Complexity:} The algorithm takes polynomial time to create directed graph and then to compute topological sort. Its complexity is $\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ ( $|\mathsf{\canA_{att}}|$ + $|\mathsf{\canAUG_{att}}|$ $\times$ $|\effectiveug|$ ).
% The additional preprocessing will require to create the requires $vset$ which takes $\mathcal{O}$($\sum_{att \in \ATTR}$$|\SCOPE_{att}|$). Therefore, the complexity is $\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ $|\canAUG_{att}|$ $\times$ $|\effectiveug|$)
%Algorithm \ref{alg:algo-su-2} describes the polynomial time algorithm.

%\input{Sections/algo-sa-1sr}

It should be noted that \miniGURANGZ scheme is a subproblem of \miniGURANGO scheme where the preconditions are restricted with only the same attribute. Henceforth, algorithms for \miniGURANGO scheme can also give plan for \miniGURANGZ scheme also if certain rules from $\mathsf{canAddU}_{att}$ and $\mathsf{canAddUG}_{att}$ are removed. Therefore the complexity for such algorithms will be similar to $\mathrm{[}\miniGURANGO{-}\overline{N}\mathrm{]}$ and $\mathrm{[}\miniGURANGO{-}\overline{D},\SR\mathrm{]}$ schemes.
\begin{col}\label{}
Reachability query types \RPSUPER and \RPSAME for scheme $\mathrm{[}\miniGURANGZ{-}\overline{N}\mathrm{]}$ and $\mathrm{[}\miniGURANGZ{-}\overline{D},\SR\mathrm{]}$ is P.
\end{col}




==> Sections/Irrelevant/su-1+-n.tex <==
The algorithm for \RPSUPER for $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ scheme is an extension to Algorithm \ref{algo:sup-1n}, where besides change in the attributes of user and its effective groups, $\Assign$ rules are also checked to get new memberships.  

\iffalse
We will now discuss \RPSUPER for $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ scheme for which we propose Algorithm \ref{algo:sup-1+n}. This algorithm is an extension to Algorithm \ref{algo:sup-1n}, in which new groups can be also added to the user in addition to the change in attributes of user or effective groups. We will consider $\canA_{att}$ rules for user, $\canAUG_{att}$ for groups and $\Assign$ rules to add new groups to the user. The algorithm continues to add new groups unless query is satisfied or no more groups can be added.
\fi
%The outer while loop in the algorithm adds new user groups or attributes to the user or user groups based on the additions done during previous iterations.%Further, with the negation restriction, we can add as many user groups and attributes without need to remove existing values.

\begin{thm}\label{}
Reachability query type \RPSUPER for scheme $\mathrm{[\miniGURANGOP{-}\overline{N}]}$ is P.
\end{thm}
\begin{proof}
Detailed algorithm is discussed in appendix.
%Algorithm \ref{algo:sup-1+n} describes the polynomial time algorithm.
\end{proof}

\noindent
\iffalse
\textbf{Correctness:} The algorithm involves a minor change of adding new effective user groups to the user, which results in more inherited values as compared to algorithm \ref{alg:algo-su-1-n}. Also, since we get all the effective user groups of the user, the maximum set of attributes are achieved.
\fi
\iffalse
\noindent
\textbf{Complexity:} With more administrative rules for assigning new user-groups, the added complexity is $\mathcal{O}$($|\mathsf{\Assign}|$ $\times$ $|\UG|$) since with every traverse in the first for loop, only one user group is added. Thus, the total complexity is $\mathcal{O}$($|\mathsf{\Assign}|$ $\times$ $|\UG|$ + ($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ $|\mathsf{\canAUG_{att}}|$ $\times$ $|\effectiveug|$ ) which is polynomial.
\fi
%The complexity is dominated by the number of times $\canA_{att}$ is traversed. If only one value is added to each attribute for all the effective user-group of the user, the complexity of Algorithm \ref{alg:algo-su-1-n} is $\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ $|\mathsf{\canA_{att}}|$ $\times$ $|\effectiveug|$ ) which is polynomial, where $|\effectiveug|$ represents the effective user-groups for the user. 

==> Sections/Irrelevant/su-1+-sr.tex <==
\smallskip

In $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ scheme, the only change required is the addition of new groups to the user. Since the precondition for adding new groups only have current direct groups as conjuncts, we can first independently calculate the effective groups of user and then run the same algorithms as discussed for $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ scheme.

\iffalse
We will now discuss \RPSUPER for $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ scheme. This algorithm adds to the algorithm for scheme \RPSUPER for $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ discussed in the previous section. In this scheme, with no deletion and single rule with direct values, we can first calculate the final set of effective user groups which can be assigned to the user. We create a separate plan for assigning new groups to the user. Once the final set of effective groups are achieved, the algorithm runs in similar manner as Algorithm \ref{algo:sup-1sr}. It should be noted that the $\Assign$ rules will only have direct user group memberships as preconditions. %Also, since we only include direct values, while getting new user-groups, we keep looping till we get the final set of effective user-groups user can get and then use these user groups to calculate the final set of effective attributes.

\fi
\begin{thm}\label{}
Reachability query type \RPSUPER for scheme $\mathrm{[\miniGURANGOP{-}\overline{D},\SR]}$ is P.
\end{thm}
\begin{proof}
Detailed algorithm for generating group plan is discussed in appendix.
%Algorithm \ref{algo:sup-1+sr} describes polynomial algorithm for group assignment plan followed by plan generated by algorithm \ref{algo:sup-1sr}.
\end{proof}

\noindent
\iffalse
\textbf{Correctness:} The only change with respect to the Algorithm \ref{alg:algo-su-2} is the assignment of new user groups before we computer the values. Hence, the proof of correctness can be similarly stated. % The algorithm involves a minor change of adding more effective user-groups to the user and giving more values as compared to algorithm \ref{alg:algo-sa-1-n}.
\fi
\iffalse
\noindent
\textbf{Complexity:} The added step to create a separate graph for group assignment plan will have complexity of $\mathcal{O}$($|\UG|$ $\times$ $|\mathsf{\Assign}|$). Therefore the total complexity is $\mathcal{O}$($|\UG|$ $\times$ $|\mathsf{\Assign}|$ + ($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ $|\canAUG_{att}|$ $\times$ $|\effectiveug|$). 
\fi

==> Sections/Irrelevant/su-1-n.tex <==
We will now discuss \RPSUPER for $\mathrm{[\miniGURANGO{-}\overline{N}]}$ scheme which can be solved in polynomial time by Algorithm \ref{algo:sup-1n}. We have extended the algorithm discussed in \miniGURANO~ \cite{jin2013reachability} to accommodate the benefits of user-group attributes assignment. Since, this scheme doesn't include negation as conjunct in preconditions, administrative rules cannot specify addition of new attributes based on the absence of some values. Therefore, current values of user or user-groups are not required to be removed, which precludes the need for investigating any $\canD_{att}$ and $\canDUG_{att}$ rules. The algorithm starts with the current set of attribute values for user and its member groups and traverse $\canA_{att}$ and $\canAUG_{att}$ rules to add as many values to the attributes of user and its effective user groups. As \miniGURANGO scheme obviates user to group membership change, we do not need to consider $\Assign$ and $\Remove$ administrative rules. The while loop (line 4--16) terminates when either the query is satisfied or when no other values can be added from the rules in $\canA_{att}$ and $\canAUG_{att}$. When a new attribute is added, its corresponding administrative request is appended to the reachability plan $plan$. If the query is satisfied, the algorithm returns the corresponding reachability plan or returns false stating that the query is unsatisfiable and user will not achieve desired effective attributes as mentioned in query.


%After all attributes assignment are made, the algorithm returns a reachability plan if the query is satisfied or return false stating that the query is unsatisfiable and user will not achieve desired effective attributes in the query.

 %The traversal of all relevant administrative rules will give the maximum set of effective attributes the user will get. The assignment is done until the query is satisfied or all rules have been traversed and no more values can be added to either user or its effective groups. Also in relaxed query type (\RPSUPER), we can add as many values even the query gets satisfied in some earlier state.


\begin{thm}\label{}
Reachability query type \RPSUPER for scheme $\mathrm{[\miniGURANGO{-}\overline{N}]}$ is P.
\end{thm}
\begin{proof}
Algorithm \ref{algo:sup-1n} provides the polynomial time algorithm.
\end{proof}
%\subsection{\miniGURANGOB Schemes}
%\include{Sections/algo-su-1}

\noindent
\iffalse
\textbf{Correctness:} If algorithm \ref{alg:algo-su-1-n} returns a plan, it can be empty, with query $q$ satisfied in $\gamma$ or there must exists $\canA_{att}$ rules for each adminsitrative action in $plan$. If algorithm return false, no $plan$ exists. We use contradiction to prove the correctness. Let us assume a $plan$ = $\mathrm{\langle}$a$_1$, a$_2$, a$_3$ .... a$_n$$\mathrm{\rangle}$  exists, which is not detected by this algorithm and without loss of generality, we say action a$_k$ is not detected by this algorithm. Assuming the state before a$_k$ is $\gamma'$ and action a$_k$ is not added to $plan$ if either preconditions are not satisifed by user u or effective user-groups in state $\gamma'$ or the value added in action a$_k$ already exists in state $\gamma'$. In both of these cases, a$_k$ cannot exist.  %Also, the algorithm checks through each user group in the effective user groups of the user, to add values. Hence all the values which can be added directly or through user-group memberships should be included by the algorithm.
 Further, the algorithm stops because the number of administrative rules and the attribute values are bounded.
\fi
\smallskip
\noindent
\textbf{Complexity:} The complexity is determined by the number of times rules in $\canA_{att}$ and $\canAUG_{att}$ are traversed. If only one value is added to each attribute for the user and its effective groups, the complexity of Algorithm \ref{algo:sup-1n} is $\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ ( $|\mathsf{\canA_{att}}|$ + $|\mathsf{\canAUG_{att}}|$ $\times$ $|\effectiveug|$ ), where $|\canA_{att}|$ and $|\canAUG_{att}|$ represents number of the administrative rules for user and its effective groups respectively and $|\effectiveug|$ represents the number of effective groups of the user. Clearly, the complexity of algorithm is polynomial. 

==> Sections/Irrelevant/su-1-sr.tex <==
We will now consider another restricted instance for \miniGURANGO, $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ for which we extend \miniGURANO~algorithm discussed in \cite{jin2013reachability}. The scheme has two restrictions, $\mathrm{\overline{D}}$ which removes the need to consider delete administrative rules in relations $\canD_{att}$ and $\canDUG_{att}$, and \SR~restriction which allows single preconditions for a pair of attribute value, with only direct values as conjuncts in preconditions. The \SR~restriction results in rules which can be either satisfied by user or its effective groups but not both. The algorithm checks the final set of values required to satisfy the reachability query and find the $\canA_{att}$ and $\canAUG_{att}$ rules to add those values. Further to add the values in precondition, it may in-turn need some other rules and values and so on. Therefore, algorithm traverses backward to find the set of values required to satisfy the query. Since the values can be achieved by user directly or from any of its effective groups, this backward search is done for user and all its effective groups. If no rule is available in both $\canA_{att}$ and $\canAUG_{att}$ relations to add a required value, the algorithm returns false. With single rule direct values restriction, backward search only limits to direct values assigned which reduces the search space. Also, if certain negative preconditions are present in starting state $\gamma'$, query cannot be satisfied, since we don't consider delete operations. If some negative conditions are introduced in later stages, addition of values should be ordered based on mutual dependencies. We create a directed graph which reflects dependencies of attribute values. This graph includes vertices as attribute value pair and directed edges if one pair is required to get the other pair. Finally, topological sort is generated which gives order in which attributes should be added to user or its groups. The plan to satisfy query will be the set of administrative request in order of topological sort.

\iffalse
We will now discuss another instance for \miniGURANGO for which we provide polynomial time Algorithm \ref{algo:sup-1sr} which is an extension to \miniGURANO~algorithm discussed in \cite{jin2013reachability}. The scheme defined as $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ has two restrictions, $\mathrm{\overline{D}}$ which removes the need to consider delete administrative rules in relations $\canD_{att}$ and $\canDUG_{att}$. Also we consider \SR~restriction which allows single preconditions for a pair of attribute value, with only direct values as conjuncts in preconditions. Therefore, the rules can be satisfied either by user or by any of its effective groups. The algorithm checks the final set of values required to satisfy the reachability query and find the $\canA_{att}$ and $\canAUG_{att}$ rules to add those values. Also to add the values in precondition, it may in-turn need some other rules and values and so on. Therefore, algorithm traverses backward to find the set of values required to satisfy the query. Since the values can be achieved by user directly or from any of its effective groups, this backward search is done for user and all its effective groups. If no rule is available in both $\canA_{att}$ and $\canAUG_{att}$ relations to add a required value, the algorithm returns false.  With single rule direct values restriction, the backward search only limits to the direct values assigned which reduces the search space.  Further, if certain negative preconditions are present in starting state $\gamma'$, query cannot be satisfied, since we don't consider delete operations. If some negative conditions are introduced in later stages, addition of values should be ordered based on mutual dependencies. We create a directed graph which reflects dependencies of attribute values. This graph includes vertices as attribute value pair and directed edges if one pair is required to get the other pair. Finally, topological sort is generated which gives the order in which attributes should be added to user or its effective groups. The plan to satisfy the query will be the set of administrative request in order of the topological sort.
\fi
\begin{thm}\label{}
Reachability query type \RPSUPER for scheme $\mathrm{[\miniGURANGO{-}\overline{D},\SR]}$ is P.
\end{thm}
\begin{proof}
Detailed algorithm is discussed in appendix.
%Algorithm \ref{algo:sup-1sr} describes the polynomial time algorithm.
\end{proof}
%\noindent
\iffalse
\textbf{Correctness:}
An empty plan is returned when query $q$ is satisfied in state $\gamma$. If the plan is non-empty, we assume a
$plan$ = $\mathrm{\langle}$a$_1$, a$_2$, a$_3$ .... a$_n$$\mathrm{\rangle}$ is returned. To prove that it is a valid plan, we first prove action a$_1$ is allowed. This action can be done on the user or any of the effective user-groups. To execute it, the preconditions should be satisfied in state $\gamma$. The for loop in line 13 only stops when $ppre_u$ and $ppre_{ug}$ doesn't change. It means the positive preconditions for all the $toadd^\prime_e$ are already in $ppre$ for user or user-groups or the current state i.e $\gamma$. Since a$_1$ is first action, it is satisfied in $\gamma$. The negative preconditions should also be satisfied in $\gamma$, stated by line 37. The next actions for user or user-group are satisfied either by the current state or previous administrative actions.s The topological graph is constructed considering all attribute-value pairs for user and all effective user-groups which would give set of actions either directly on user or on user-groups. \fi
\iffalse
\smallskip
\noindent
\textbf{Complexity:} The algorithm takes polynomial time to create directed graph and then to compute topological sort. Its complexity is $\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ ( $|\mathsf{\canA_{att}}|$ + $|\mathsf{\canAUG_{att}}|$ $\times$ $|\effectiveug|$ ). \fi
%$\mathcal{O}$(($\sum_{att \in \ATTR}|\SCOPE_{att}|$) $\times$ $|\canAUG_{att}|$ $\times$ $|\effectiveug|$).


==> Tables/Irrelevant/table_tab_3.tex <==
\begin{table}[t]
\centering
\caption{ Administrative Relations }
\resizebox{\columnwidth}{!}{%
\label{tab gura}
\begin{tabular}{@{}lllll@{}}

\toprule
\iffalse
\multicolumn{5}{l}{\textbf{Administrative Roles and Expressions}}\\
[\defaultaddspace]
\multicolumn{5}{l}{-- AR : a finite set of administrative roles}      \\
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}}-- EXPR(UA) : a finite set of prerequisite expressions composed of user attribute \\ \;\; functions as defined in section \ref{s.uaa} and \ref{s.ugaa}  \end{tabular}}\\
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}}-- EXPR(UA $\cup$ UG) : a finite set of prerequisite expressions composed of user \\ \;\; attribute  functions and user groups as defined in section \ref{s.uga} \end{tabular}}\\
\\
\multicolumn{5}{l}{\textbf{Administrative Model}}\\
[\defaultaddspace]
\fi
\multicolumn{5}{l}{ AR : a finite set of administrative roles}\\
\multicolumn{5}{l}{ C : a finite set of prerequisite conditions as defined in \GURAG model}\\
\toprule
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{User Attribute Assignment} and \textbf{User Group Attribute Assignment}:%\textbf{UAA} \&  \textbf{UGAA:}
\\ 
\;\;For each ${att}$ in \ATTR,  \end{tabular}}
 \\%[1mm] \midrule
\multicolumn{5}{l}{\centerline{$\mathsf{canAdd}_{att} \subseteq \AR \times \C \times \SCOPE_{att}$}} \\[1mm]


\multicolumn{5}{l}{\centerline{$\mathsf{canDelete}_{att} \subseteq \AR \times \C \times \SCOPE_{att}$}} \\[1mm]
%\midrule
%\midrule
\multicolumn{5}{l}{ \textbf{User to User Group Assignment}:} \\[1mm]
%\midrule





\multicolumn{5}{l}{\centerline{$ \mathsf{canAssign} \subseteq \AR \times \C \times \UG $}}
\\ [1mm]
\multicolumn{5}{l}{\centerline{$ \mathsf{canRemove} \subseteq \AR \times \C \times \UG $}}
\\ [1mm]

\toprule
\end{tabular}
}
\end{table} 

==> Tables/Irrelevant/table_tab_4.tex <==
\begin{table*} [t] \footnotesize
\centering
\caption{State Transition Function $\delta: \Gamma \times \REQ \rightarrow \Gamma$}
\label{table:transition}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|p{.18\textwidth}|p{.75\textwidth}|} \hline
%\multicolumn{2}{|p{.93\textwidth}|}{
%In this table:
%}\\
% \multicolumn{2}{|p{.93\textwidth}|}{
% (1) We assume that $\mathrm{\langle}$$u$, $att$, $val$$\mathrm{\rangle}$
% $\in$ \UAAN$_{\gamma_1}$ for atomic-valued attributes and
% $\mathrm{\langle}$$u$, $att$, $setval$$\mathrm{\rangle}$
% $\in$ \UAAN$_{\gamma_1}$ for set-valued attributes.}\\

\multicolumn{2}{|p{.93\textwidth}|}{
(1) Let $\gamma_1$ and $\gamma_2$ be the source and target state respectively.
In all requests in the first column, $ar$ $\in$ \AR, $u$ $\in$ \U, $ug$ $\in$ \UG, $att$ $\in$ \ATTR, $val'$ $\in$ ${\SCOPE_{att}}$, $ug' \in \UG$.
}\\

\multicolumn{2}{|p{.93\textwidth}|}{
(2)
$\Evaluate_u$ : \U $\times$ \C $\times$ $\Gamma$
$\rightarrow$ \{\true, \false\}, returns \true\xspace
if user $u\in U$ satisfies precondition $c\in \C$ in state $\gamma\in\Gamma$, else \false .
}
\\
\multicolumn{2}{|p{.93\textwidth}|}{
(3)
$\Evaluate_{ug}$ : \UG $\times$ \C $\times$ $\Gamma$
$\rightarrow$ \{\true, \false\}, returns \true\xspace
if user group $ug\in UG$ satisfies precondition $c\in \C$ in state $\gamma\in\Gamma$, else \false .
}
\\
\multicolumn{2}{|p{.93\textwidth}|}{
(4)
$\Evaluate_{u\?{12}-\?{12}ug}$ : \U $\times$ \C $\times$ $\Gamma$
$\rightarrow$ \{\true, \false\}, returns \true\xspace
if user $u\in U$ satisfies precondition $c\in \C$ in state $\gamma\in\Gamma$, else \false .
}
\\


 \hline\hline

\textbf{Request} & \textbf{Target State}\\ \hline
\iffalse
\multirow{3}{*}{$\mathsf{assign}$($ar$, $u$, $att$, $val^\prime$)} & \textbf{if} $\exists$
$\mathrm{\langle}ar,~c,~val\mathrm{\rangle}$ $\in$ $\mathsf{can\_assign}_{att}$
$\wedge$ $\Evaluate(u,~c,~\gamma_1)$ \\
&  \hspace{5pt}\textbf{then}  transition to target state $\gamma_2$ where:
$\UAAN_{\gamma_2}$ = $\UAAN_{\gamma_1}$
$\backslash$ $\mathrm{\langle}u, att, val\mathrm{\rangle}$
$\cup$ $\mathrm{\langle}u, att, val^\prime\mathrm{\rangle}$  \\
&   \textbf{else} remain in $\gamma_1$ \\ \hline
\fi

\multirow{4}{*}{$\mathsf{add}$($ar$, $u$, $att$, $val^\prime$)
}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~val'\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$
$\wedge$ $\Evaluate_u(u,~c,~\gamma_1)$\\

& \hspace{5pt} \textbf{then} transition to target state $\gamma_2$ such
that
$\UAAN_{\gamma_2}$ = $\UAAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$u$, $att$ ,
$att_{\gamma_{1}}(u)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$u$, $att$,
$att_{\gamma_{2}}(u)$$\mathrm{\rangle}$\\
& \hspace{5pt} where
%$att(u)=setval$ in state $\gamma_1$ and
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$ $\cup$ \{$val^\prime$\},
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$,
$\directug_{\gamma_{2}}(u)$ = $\directug_{\gamma_{1}}(u)$
\\
% /*$setval$ is the attribute value assignment in $\gamma_1$*/\\

& \textbf{else}
remain in $\gamma_1$\\ \hline

\multirow{4}{*}{$\mathsf{delete}$($ar$, $u$, $att$, $val^\prime$)}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~val'\mathrm{\rangle}$ $\in$ $\mathsf{canDelete}_{att}$
$\wedge$
$\Evaluate_u(u,~c,~\gamma_1)$ \\

& \hspace{5pt} \textbf{then} transition to target state $\gamma_2$ where:
$\UAAN_{\gamma_2}$ = $\UAAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$u$, $att$ ,
$att_{\gamma_{1}}(u)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$u$, $att$,
$att_{\gamma_{2}}(u)$$\mathrm{\rangle}$ \\
& \hspace{5pt} where
%$att(u)=setval$ in state $\gamma_1$ and
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$ $\backslash$ \{$val^\prime$\},
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$,
$\directug_{\gamma_{2}}(u)$ = $\directug_{\gamma_{1}}(u)$
\\
& \textbf{else} remain in $\gamma_1$ \\ \hline

\multirow{4}{*}{$\mathsf{add}$($ar$, $ug$, $att$, $val^\prime$)
}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~val'\mathrm{\rangle}$ $\in$ $\mathsf{canAdd}_{att}$
$\wedge$ $\Evaluate_{ug}(ug,~c,~\gamma_1)$\\

& \hspace{5pt} \textbf{then} transition to state $\gamma_2$ where:
$\UGAAN_{\gamma_2}$ = $\UGAAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$ug$, $att$ ,
$att_{\gamma_{1}}(ug)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$ug$, $att$,
$att_{\gamma_{2}}(ug)$$\mathrm{\rangle}$\\
& \hspace{5pt}
where
%$att(u)=setval$ in state $\gamma_1$ and
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$ $\cup$ \{$val^\prime$\},
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$,
$\directug_{\gamma_{2}}(u)$ = $\directug_{\gamma_{1}}(u)$
\\
% /*$setval$ is the attribute value assignment in $\gamma_1$*/\\

& \textbf{else}
remain in $\gamma_1$\\ \hline

\multirow{4}{*}{$\mathsf{delete}$($ar$, $ug$, $att$, $val^\prime$)}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~val'\mathrm{\rangle}$ $\in$ $\mathsf{canDelete}_{att}$
$\wedge$
$\Evaluate_{ug}(ug,~c,~\gamma_1)$ \\

& \hspace{5pt} \textbf{then} transition to state $\gamma_2$ where:
$\UGAAN_{\gamma_2}$ = $\UGAAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$ug$, $att$ ,
$att_{\gamma_{1}}(ug)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$ug$, $att$,
$att_{\gamma_{2}}(ug)$$\mathrm{\rangle}$\\
& \hspace{5pt}
where
%$att(u)=setval$ in state $\gamma_1$ and
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$ $\backslash$ \{$val^\prime$\},
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$,
$\directug_{\gamma_{2}}(u)$ = $\directug_{\gamma_{1}}(u)$
\\
& \textbf{else} remain in $\gamma_1$ \\ \hline

\multirow{4}{*}{$\mathsf{assign}$($ar$, $u$, $ug'$)
}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~ug'\mathrm{\rangle}$ $\in$ $\mathsf{canAssign}$
$\wedge$ $\Evaluate_{u\?{12}-\?{12}ug}(u,~c,~\gamma_1)$\\

& \hspace{5pt} \textbf{then} transition to state $\gamma_2$ where:
$\UGAN_{\gamma_2}$ = $\UGAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$u$,
$\directug_{\gamma_1}(u)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$u$,
$\directug_{\gamma_2}(u)$$\mathrm{\rangle}$\\
& \hspace{5pt} where
%$\directug(u)=setval$ in state $\gamma_1$ and
$\directug_{\gamma_2}(u)$ = $\directug_{\gamma_1}(u)$ $\cup$ \{$ug^\prime$\},
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$ ,
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$
\\
% /*$setval$ is the attribute value assignment in $\gamma_1$*/\\

& \textbf{else}
remain in $\gamma_1$\\ \hline

\multirow{4}{*}{$\mathsf{remove}$($ar$, $u$, $ug'$)}
&
\textbf{if} $\exists$ $\mathrm{\langle}ar,~c,~ug'\mathrm{\rangle}$ $\in$ $\mathsf{canRemove}$
$\wedge$
$\Evaluate_{u\?{12}-\?{12}ug}(u,~c,~\gamma_1)$ \\

& \hspace{5pt} \textbf{then} transition to state $\gamma_2$ where:
$\UGAN_{\gamma_2}$ = $\UGAN_{\gamma_1}$ $\backslash$ $\mathrm{\langle}$$u$,
$\directug_{\gamma_1}(u)$$\mathrm{\rangle}$ $\cup$ $\mathrm{\langle}$$u$,
$\directug_{\gamma_2}(u)$$\mathrm{\rangle}$\\
& \hspace{5pt} where
%$\directug(u)=setval$ in state $\gamma_1$ and
$\directug_{\gamma_2}(u)$ = $\directug_{\gamma_1}(u)$ $\backslash$ \{$ug^\prime$\},
$att_{\gamma_{2}}(ug)$ = $att_{\gamma_{1}}(ug)$ ,
$att_{\gamma_{2}}(u)$ = $att_{\gamma_{1}}(u)$
\\
& \textbf{else} remain in $\gamma_1$ \\ \hline
\end{tabular}
\end{table*}

